RobustPeriod: Time-Frequency Mining for Robust Multiple Periodicity Detection

Periodicity detection is a crucial step in time series tasks, including monitoring and forecasting of metrics in many areas, such as IoT applications and self-driving database management system. In many of these applications, multiple periodic components exist and are often interlaced with each other. Such dynamic and complicated periodic patterns make the accurate periodicity detection difficult. In addition, other components in the time series, such as trend, outliers and noises, also pose additional challenges for accurate periodicity detection. In this paper, we propose a robust and general framework for multiple periodicity detection. Our algorithm applies maximal overlap discrete wavelet transform to transform the time series into multiple temporal-frequency scales such that different periodic components can be isolated. We rank them by wavelet variance, and then at each scale detect single periodicity by our proposed Huber-periodogram and Huber-ACF robustly. We rigorously prove the theoretical properties of Huber-periodogram and justify the use of Fisher's test on Huber-periodogram for periodicity detection. To further refine the detected periods, we compute unbiased autocorrelation function based on Wiener-Khinchin theorem from Huber-periodogram for improved robustness and efficiency. Experiments on synthetic and real-world datasets show that our algorithm outperforms other popular ones for both single and multiple periodicity detection.

==> 8_Supple_rPeriod.tex <==
% \def\year{2020}\relax
% %File: formatting-instruction.tex
% \documentclass[letterpaper]{article} % DO NOT CHANGE THIS

% %\usepackage[]{algorithm2e}
% \usepackage{algorithm}  
% \usepackage{algorithmic}  
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm  
% \renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm 

% % \usepackage{aaai20}  % DO NOT CHANGE THIS
% \usepackage{times}  % DO NOT CHANGE THIS
% \usepackage{helvet} % DO NOT CHANGE THIS
% \usepackage{courier}  % DO NOT CHANGE THIS
% \usepackage[hyphens]{url}  % DO NOT CHANGE THIS
% \usepackage{graphicx} % DO NOT CHANGE THIS
% \urlstyle{rm} % DO NOT CHANGE THIS
% \def\UrlFont{\rm}  % DO NOT CHANGE THIS
% \usepackage{graphicx}  % DO NOT CHANGE THIS
% \frenchspacing  % DO NOT CHANGE THIS
% \setlength{\pdfpagewidth}{8.5in}  % DO NOT CHANGE THIS
% \setlength{\pdfpageheight}{11in}  % DO NOT CHANGE THIS
% %\nocopyright
% %PDF Info Is REQUIRED.
% % For /Author, add all authors within the parentheses, separated by commas. No accents or commands.
% % For /Title, add Title in Mixed Case. No accents or commands. Retain the parentheses.


% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{amsfonts}
% \usepackage{amssymb}
% %\usepackage{cite}

% %\usepackage{textcomp}
% %\usepackage{xcolor}
% \usepackage{multirow}
% %\usepackage{multicol}

% \newtheorem{proposition}{Proposition}
% \newtheorem{theorem}{Theorem}






%  \pdfinfo{
% /Title (tfPeriod:  time-frequency mining for robust multiple periodicities detection)
% /Author (xxx, ...)
% } %Leave this	
% % /Title ()
% % Put your actual complete title (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case
% % Leave the space between \Title and the beginning parenthesis alone
% % /Author ()
% % Put your actual complete list of authors (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case. 
% % Each author should be only by a comma. If the name contains accents, remove them. If there are any LaTeX commands, 
% % remove them. 
% % DISALLOWED PACKAGES
% % \usepackage{authblk} -- This package is specifically forbidden
% % \usepackage{balance} -- This package is specifically forbidden
% % \usepackage{caption} -- This package is specifically forbidden
% % \usepackage{color (if used in text)
% % \usepackage{CJK} -- This package is specifically forbidden
% % \usepackage{float} -- This package is specifically forbidden
% % \usepackage{flushend} -- This package is specifically forbidden
% % \usepackage{fontenc} -- This package is specifically forbidden
% % \usepackage{fullpage} -- This package is specifically forbidden
% % \usepackage{geometry} -- This package is specifically forbidden
% % \usepackage{grffile} -- This package is specifically forbidden
% % \usepackage{hyperref} -- This package is specifically forbidden
% % \usepackage{navigator} -- This package is specifically forbidden
% % (or any other package that embeds links such as navigator or hyperref)
% % \indentfirst} -- This package is specifically forbidden
% % \layout} -- This package is specifically forbidden
% % \multicol} -- This package is specifically forbidden
% % \nameref} -- This package is specifically forbidden
% % \natbib} -- This package is specifically forbidden -- use the following workaround:
% % \usepackage{savetrees} -- This package is specifically forbidden
% % \usepackage{setspace} -- This package is specifically forbidden
% % \usepackage{stfloats} -- This package is specifically forbidden
% % \usepackage{tabu} -- This package is specifically forbidden
% % \usepackage{titlesec} -- This package is specifically forbidden
% % \usepackage{tocbibind} -- This package is specifically forbidden
% % \usepackage{ulem} -- This package is specifically forbidden
% % \usepackage{wrapfig} -- This package is specifically forbidden
% % DISALLOWED COMMANDS
% % \nocopyright -- Your paper will not be published if you use this command
% % \addtolength -- This command may not be used
% % \balance -- This command may not be used
% % \baselinestretch -- Your paper will not be published if you use this command
% % \clearpage -- No page breaks of any kind may be used for the final version of your paper
% % \columnsep -- This command may not be used
% % \newpage -- No page breaks of any kind may be used for the final version of your paper
% % \pagebreak -- No page breaks of any kind may be used for the final version of your paperr
% % \pagestyle -- This command may not be used
% % \tiny -- This is not an acceptable font size.
% % \vspace{- -- No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% % \vskip{- -- No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference
% \setcounter{secnumdepth}{0} %May be changed to 1 or 2 if section numbers are desired.
% % The file aaai20.sty is the style file for AAAI Press 
% % proceedings, working notes, and technical reports.
% %
% \setlength\titlebox{2.5in} % If your paper contains an overfull \vbox too high warning at the beginning of the document, use this
% % command to correct it. You may not alter the value below 2.5 in




% %\title{tfPeriod: Robust Time-Frequency Mining for Multiple Periodicities Detection}
% \title{SUPPLEMENTAL MATERIAL TO\\tfPeriod: Robust Time-Frequency Mining for Periodicity Detection and Estimation}

% %\title{AAAI Press Formatting Instructions \\for Authors Using \LaTeX{} --- A Guide }
% %Your title must be in mixed case, not sentence case. 
% % That means all verbs (including short verbs like be, is, using,and go), 
% % nouns, adverbs, adjectives should be capitalized, including both words in hyphenated terms, while
% % articles, conjunctions, and prepositions are lower case unless they
% % directly follow a colon or long dash

% \author{xxx, yyy\\ 
% Anonymous Affiliation\\
% Address of Anonymous Affiliation\\
% \{xxx,yyy\}@xxx.xxx}

% % \author{xxx, yyy\\ 
% % Machine Intelligence Technology, Alibaba Group\\
% % Bellevue, Washington 98004, USA\\
% % \{xxx\}@alibaba-inc.com}

% %\author{Written by AAAI Press Staff\textsuperscript{\rm 1}\thanks{Primarily Mike Hamilton of the Live Oak Press, LLC, with help from the AAAI Publications Committee}\\ \Large \textbf{AAAI Style Contributions by
% %Pater Patel Schneider,} \\ \Large \textbf{Sunil Issar, J. Scott Penberthy, George Ferguson, Hans Guesgen}\\ % All authors must be in the same font size and format. Use \Large and \textbf to achieve this result when breaking a line
% %\textsuperscript{\rm 1}Association for the Advancement of Artificial Intelligence\\ %If you have multiple authors and multiple affiliations
% %% use superscripts in text and roman font to identify them. For example, Sunil Issar,\textsuperscript{\rm 2} J. Scott Penberthy\textsuperscript{\rm 3} George Ferguson,\textsuperscript{\rm 4} Hans Guesgen\textsuperscript{\rm 5}. Note that the comma should be placed BEFORE the superscript for optimum readability
% %2275 East Bayshore Road, Suite 160\\
% %Palo Alto, California 94303\\
% %publications20@aaai.org % email address must be in roman text type, not monospace or sans serif
% %}
%  \begin{document}
% \maketitle




% Regarding the supplementary PDF file:

% We encourage submitting code for reproducibility, but again, it is important that this does not identify you or your institution
% nice examples, additional figures
% additional results / experiments, proofs that do not provide essential insights for understanding the contribution of the paper
% proofs or other supplement matter are an important part of the contribution, their essential elements should be included in the main paper. 
% \section{Detailed Experiments Setup}
% xxx
 
% \newpage
% \input{7_Appendix.tex}

\section{Appendix}
% \section{ADMM for Huber-Periodogram and Complexity Analysis}
\subsection{Implementation Overview}
In this section, we describe the implementation of the proposed robustPeriod algorithm. 

Our robustPeriod algorithm is implemented with Python, where 
the H-P filter is based on statsmodels\footnote{Seabold, Skipper, and Josef Perktold. “statsmodels: Econometric and statistical modeling with python.” Proceedings of the 9th Python in Science Conference. 2010.},
the MODWT is based on the PyWavelets\footnote{Gregory R. Lee, Ralf Gommers, Filip Wasilewski, Kai Wohlfahrt, Aaron O’Leary (2019). PyWavelets: A Python package for wavelet analysis. Journal of Open Source Software, 4(36), 1237, https://doi.org/10.21105/joss.01237.}, 
the DFT/IDFT based on Scipy\footnote{Virtanen, P., Gommers, R., Oliphant, T.E. et al. SciPy 1.0: fundamental algorithms for scientific computing in Python. Nat Methods (2020). https://doi.org/10.1038/s41592-019-0686-2.}, and 
the peak detection of ACF is based on signal.find\_peaks in Scipy.

For the parameters of different components in robustPeriod algorithm, we adopt a fixed configurations for all experiments in the paper. It works quit well as shown in experiment section in the paper, which also makes our robustPeriod widely deployed in different  applications in Alibaba. 
Specifically, the time series is normalized by mean and variance in H-P filter and its $\lambda$ is set as $10^{-6}$ in Eq.~\eqref{eq:hp_trend}. The MODWT is set as Daubechies-4. In the Huber-Periodogram, the result of $\boldsymbol{\phi} \boldsymbol{\beta} -  \mathbf{x}$ in Eq.~\eqref{eq:Periodogram_final} is normalized by mean and variance before the operation of Huber function where the threshold in Huber is set as $\zeta=1$ in Eq.~\eqref{eq:huber_loss}, and the threshold in Fisher test in Section~\ref{sec:RobustFisher} is set as $\alpha=10^{-10}$. In the peak detection of normalized ACF in Section~\ref{sec:RobustACF}, we set the threshold as 0.5. The normalization in H-P filter and Huber function makes the parameter setting simple and can be used in a wide of time series. 

Note that for most parts of the proposed robustPeriod algorithm, their implementation is straightforward based on the formulation in the paper, except the solution of the proposed Huber-Periodogram which is described in details in the following subsection.

\subsection{Implementation of Huber-Periodogram}
\subsubsection{ADMM formulation}
We apply ADMM to solve the proposed Huber-Periodogram. Firstly we reformulate the optimization problem of Huber-Periodogram in Eq.~\eqref{eq:Periodogram_final} as
\begin{eqnarray}\label{eq:Periodogram_admm}
& \min &   \gamma_{\zeta}^{hub} ( \mathbf{z})\\
& ~~~\text{s.t.}\quad & \boldsymbol{\phi} \boldsymbol{\beta} -  \mathbf{x}  = \mathbf{z}
\end{eqnarray}
Then we can obtain the augmented Lagrangian as
\begin{equation}\label{eq:Lagrangian} \notag
L_{\rho}(\boldsymbol{\beta},\mathbf{z},\mathbf{v}) = 
\gamma_{\zeta}^{hub}(\mathbf{z}) +
\mathbf{v}^T ( \boldsymbol{\phi} \boldsymbol{\beta} -  \mathbf{x}  - \mathbf{z}) + \frac{\rho}{2} || \boldsymbol{\phi} \boldsymbol{\beta} -  \mathbf{x}  - \mathbf{z}||_2^2
\end{equation}
where $\mathbf{v}$ is the dual variable, and $\rho$ is the penalty parameter.
Following the ADMM procedure~\cite{boyd2011distributed} and taking proximal operator for huber function $\gamma_{\zeta}^{hub} ( \mathbf{z})$~\cite{Parikh2014}, we can obtain the updating steps as
\begin{align} % \label{eq:admm}
\boldsymbol{\beta}^{k+1} ={}&  (\boldsymbol{\phi}^T \boldsymbol{\phi} )^{-1} \boldsymbol{\phi}^T (\mathbf{z}^k+\mathbf{x}-\mathbf{u}^k)\label{eq:admm1}\\
\begin{split} 
\mathbf{z}^{k+1} ={}& \frac{\rho}{1+\rho}\left( \boldsymbol{\phi} \boldsymbol{\beta}^{k+1} + \mathbf{u}^{k}  - \mathbf{x} \right) +  \\
 & \frac{1}{1+\rho}S_{\frac{\zeta(1+\rho)}{\rho}}\left( \boldsymbol{\phi} \boldsymbol{\beta}^{k+1} + \mathbf{u}^{k}  - \mathbf{x}  \right) 
\end{split}\label{eq:admm2}\\
\mathbf{u}^{k+1} ={}& \mathbf{u}^{k} +  \boldsymbol{\phi} \boldsymbol{\beta}^{k+1} - \mathbf{z}^{k+1}- \mathbf{x}  \label{eq:admm3}
\end{align}
where $\mathbf{u}=(1/\rho)\mathbf{v}$ is the scaled dual variable to make the formulation more convenient.
The soft thresholding operation ${S}_{\rho}(x)$ in $\mathbf{z}-$minimization step can be efficiently calculated by %${S}_{\rho}(x) = (1-\rho/|x|)_{+}x$.
\begin{equation}\label{eq:soft_thresholding} 
{S}_{\rho}(x) =
\begin{cases} 
0,       & |x| \leq \rho\\
x- \rho \text{sgn}(x), & |x| > \rho
\end{cases}
\end{equation}


For the termination criteria, besides the maximum iteration number, we also check the primal and dual residuals in each ADMM iteration until they are small enough. Specifically, the values of primal residual $\mathbf{r}^k$ and dual residual $\mathbf{s}^k$ at $k$th iteration are calculated by
\begin{align}\label{eq:primal:residual}
\|\mathbf{r}^k\|_2 &= \|\boldsymbol{\phi} \boldsymbol{\beta}^{k} - \mathbf{z}^k\ - \mathbf{x}\|_2,\\
\|\mathbf{s}^k\|_2 &= \rho \|\boldsymbol{\phi}^T (\mathbf{z}^k - \mathbf{z}^{k-1})\|_2.
\end{align}
Then, $\|\mathbf{r}^k\|_2$ and $\|\mathbf{s}^k\|_2$ are checked if they are smaller than the corresponding tolerance thresholds as~\cite{boyd2011distributed}
\begin{align}   
\epsilon^{pri} &= \sqrt{N} \epsilon^{abs} + \epsilon^{rel}\max\{\|\boldsymbol{\phi} \boldsymbol{\beta}^{k}\|_2, \|\mathbf{z}^{(k)}\|_2,  \|\mathbf{x}\|_2 \},\label{eq:tol_pri} \\
\epsilon^{dual} &= \sqrt{2}\epsilon^{abs} + \epsilon^{rel}\|\rho \boldsymbol{\phi}^T \mathbf{u}^{(k)}\|_2,\label{eq:tol_dual}
\end{align}
where $\epsilon^{abs}>0$ is an absolute tolerance and $\epsilon^{rel}>0$ is a relative tolerance. 

\subsubsection{Parameter Setting}
The threshold of Huber function in~\eqref{eq:Periodogram_admm} is set as $\zeta=1$. And the threshold of soft thresholding in~\eqref{eq:admm2} is set as $\rho=1$. Both absolute tolerance $\epsilon^{abs}$and relative tolerance $\epsilon^{rel}$ are set as $10^{-4}$ in~\eqref{eq:tol_pri}, \eqref{eq:tol_dual}. Besides the termination criteria, we also set the maximum number of ADMM iteration in~\eqref{eq:admm1} to \eqref{eq:admm3} as 50. 

% where 
% The  is set as  
% % 
% % \eqref{eq:Periodogram_admm}
% % \rho} \label{eq:soft_thresholding} 
% % \label{eq:admm1}  2 3 
% % 50  

% %  {eq:tol_pri}  \label{eq:tol_dual}   \epsilon^{abs}   \epsilon^{rel}
% % A reasonable choice for the two tolerance in our case is around $10^{-3}$ to $10^{-4}$.
% % rel_par=1.,
%                         % tol_abs=1e-5,
%                         % tol_rel=1e-2):

\subsubsection{Complexity Analysis}
For the complexity of the ADMM in Huber-Periodogram, we can obtain $\mathcal{O}(N)$ computational complexity for each iteration based on Eq.~\eqref{eq:admm1} to Eq.~\eqref{eq:admm3} (note that $\boldsymbol{\phi}$ is an $N \times 2$ matrix). Furthermore, we can store the value of $(\boldsymbol{\phi}^T \boldsymbol{\phi} )^{-1} \boldsymbol{\phi}^T$ in Eq.~\eqref{eq:admm1} to save time since it is unchanged in each iteration. For required number of iteration, we can get $\epsilon$-optimal solution within $\mathcal{O}(N/\epsilon)$ iterations~\cite{boyd2011distributed}. Note that in our case, the ADMM often converges well within a few tens of iterations.










% the number of iterations required is $\mathcal{O}(N/\epsilon)$, where $\epsilon$ is the error between the solver and optimal solution. 
% For the computational complexity of each iteration (updating step) in ADMM, we can obtain $\mathcal{O}(N)$ complexity based on the updating steps in Eq.~\eqref{eq:admm1} to Eq.~\eqref{eq:admm3} (note that $\boldsymbol{\phi}$ is an $N \times 2$ matrix). 



% $\epsilon$-optimal solution within $\mathcal{O}(N/\epsilon)$ iterations


% \section{Temp}
% % \addtocounter{proposition}{2} % this is for appendix with right numbering
% sdf


% \bibliographystyle{aaai}
% %\bibliography{yourbibfile1,yourbibfile2}
% \bibliography{6_Periodicity_bibfile}

% \end{document}



==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> bakupexperiment.tex <==
% \newpage
\section{Experiments and Discussion}
% \section{Experiments and Comparisons}
We conduct experiments on synthetic datasets, public Yahoo dataset, and real-world datasets to demonstrate the effectiveness of the proposed RobustPeriod algorithm for periodicity detection and estimation.


% Many real world time series exhibit near, rather than perfect, periodicity, as a result of variation in period length (PL). robust to PL variation experiments to do...
% for detecting near-periodicity
% synthetic periodic data with varying CL and noise


\subsection{Baseline Algorithms}
For the periodicity detection, we compare RobustPeriod with the following common or stat-of-art  algorithms:
\begin{itemize}
    % \item \textbf{Fisher}~\cite{fisher1929tests,mills2011foundations}: This algorithm first calculates the vanilla periodogram, and then performs Fisher's test. If the test is passed, the final single period is $N/k$ where $k$ is the peak index of periodogram.
    
    \item \textbf{findFrequency}~\cite{hyndman2019package}: It first removes a fitted linear trend, then the spectral density function is estimated from the best fitting autoregressive model (based on the AIC). Finally, the reciprocal of the
    maximum in the spectral density function is estimated as the period length. 
    
    \item \textbf{SAZED$_{maj}$}~\cite{Toller2019}: It estimates a time series’ season length by computing six different estimates and taking a majority vote.

    \item \textbf{SAZED$_{opt}$}~\cite{Toller2019}: It estimates a time series’ season length by combining three different estimates computed on an input time series and its ten-fold self-composed autocorrelation.


    % \item \textbf{ACF-Med}: It first calculates the vanilla ACF of the time series, and detects the peaks of ACF. The median value of distances between peaks is utilized as the single period of the time series.
    
    % \item \textbf{DFT-Th}: We adopt DFT-based periodogram to estimate the power spectral density (PSD) of time series with length $N$. To find the threshold of periodogram for period candidates, we following the method in \cite{dPD_yuan2017detecting, cPD_vlachos2005Autoperiod} to permute the original signal 100 times, calculate maximum values of periodogram for each permutation, and select the 95\% percentile of the 100 maximum values as the threshold. For each index $k$ in periodogram that exceeds the threshold, the corresponding period candidate is $N/k$. 



    \item \textbf{Siegel}~\cite{Siegel1980,li2016time}: It first calculates the vanilla periodogram and then detects mulitple periods using Siegel's test. If the test is passed, the corresponding multiple periods can be obtained. 
    
    \item \textbf{AUTOPERIOD}~\cite{cPD_vlachos2005Autoperiod,Mitsa:2010:TDM:1809755}: This algorithm first select a list of period candidates based on the vanilla periodogram, and then validates them  using vanilla ACF. 
    
    \item \textbf{Wavelet-Fisher}~\cite{Abdullah:testing:periodicity}: It applies the wavelet transform to decompose the input time series into different scales, and then apply the Fisher's test to detect a single period at each scale. 
\end{itemize}
Note that the first three algorithms can only detect single period, while the other three algorithms can detect multiple periods. In the following experiments, we also adopt H-P filter to remove the trend signal for all excising algorithms otherwise their performance would degrade significantly.

% We implement DFT-Periodogram, AUTOPERIOD periodicity detection in Python.  


% \subsection{Dataset}



 
\begin{figure}[!htb] 
    \centering
    \includegraphics[width=0.8\linewidth]{plots/kdd20-simdata.pdf}
    \caption{The generated synthetic data with 3 periods. Top to bottom: 3 sine waves with period lengths ($20, 50, 100$); the summation of the 3 sine waves; simulated noise, spike \& dip outliers, and triangle trend signal; the final time series.}
\label{fig:simdata}
\vspace{-0.2cm}
\end{figure}


\begin{figure}[!htb] 
    \centering
    \includegraphics[width=0.8\linewidth]{plots/kdd20-simdata.pdf}
    \caption{The generated synthetic data with 3 periods. Top to bottom: 3 sine waves with period lengths ($20, 50, 100$); the summation of the 3 sine waves; simulated noise, spike \& dip outliers, and triangle trend signal; the final time series.}
\label{fig:realdata}
\vspace{-0.2cm}
\end{figure}

\subsection{Datasets}

real-world single-period data: CRAN dataset\cite{Toller2019} contains 82 univariate time series. The time series included in those packages span across a wide variety of application domains, ranging from economic indicators, such as employment rates or retail sales, to environmental measurements, such as pollution levels or the number of sunspots. The lengths of these time series range from 16 to 3024, and their season length ranges from 2 to 52. 


 


\subsection{Experiments and Discussion on Single-Periodicity Detection}
(TODO) refer to Table~\ref{tab:single_period_det}  













% \begin{table}[!htb] % \begin{table*}[t]
% % \footnotesize 
% \centering
% %\normalsize
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \caption{Comparisons of different single-periodicity detection algorithms on synthetic data with different noise variance $\sigma^2_n$ and outlier ratio $\eta$, as well as the real-world dataset from CRAN.}
% %\vspace{-0.1cm}
% \label{tab:single_period_det}
% \begin{tabular}{c||c|c||c|c||c|c||}
% \hline
% \multirow{2}{*}{Algorithms}  & \multicolumn{2}{|c||}{ $\sigma^2_n$ \!=\! 0.1, $\eta$ \!=\! 0.01\! } & \multicolumn{2}{|c||}{ $\sigma^2_n$ \!=\! 2, $\eta$ \!=\! 0.2\! } & \multicolumn{2}{|c||}{CRAN data} \\ \cline{2-7}
%  &  0\% & 2\% & 0\%   &  2\% & 0\% & 2\% \\ \hline
% Fisher        &  1.0 & 1.0        & 0.59 &0.59   &  0.34 & 0.39 \\ \hline
% findFrequency   &  0 & 0&        0 &0  & 0.44 & 0.44\\ \hline
% SAZED$_{opt}$   & 0  & 0.95       & 0& 0.54  & 0.55  & 0.56  \\ \hline
% {RobustPeriod} &  0.82  & 0.99     & 0.44  & 0.98   &  0.56  & 0.57  \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[!htb] % \begin{table*}[t]
% % \footnotesize 
% \centering
% %\normalsize
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \caption{Comparisons of different single-periodicity detection algorithms on synthetic data with different noise variance $\sigma^2_n$ and outlier ratio $\eta$, as well as the real-world dataset from CRAN.}
% %\vspace{-0.1cm}
% \label{tab:single_period_det}
% \begin{tabular}{c|c|c|c|c|c|c|}
% \hline
% \multirow{3}{*}{Algorithms} & \multicolumn{2}{|c|}{\multirow{2}{*}{\!Synthetic Data\!}} & \multicolumn{2}{|c|}{\multirow{2}{*}{\!Synthetic Data\!}} & \multicolumn{2}{|c|}{\multirow{2}{*}{CRAN}} \\
%                   & \multicolumn{2}{|c|}{\!$\sigma^2_n$ \!=\! 0.1, $\eta$ \!=\! 0.01\!}                  & \multicolumn{2}{|c|}{\!$\sigma^2_n$ \!=\! 2, $\eta$ \!=\! 0.2\!}    & \multicolumn{2}{|c|}{Data}      \\ \cline{2-7}    
%  &  0\% & 2\% & 0\%   &  2\% & 0\% & 2\% \\ \hline\hline
% Fisher        &  1.0 & 1.0        & 0.59 &0.59   &  0.34 & 0.39 \\ \hline
% findFrequency   &  0 & 0&        0 &0  & 0.44 & 0.44\\ \hline
% SAZED$_{opt}$   & 0  & 0.95       & 0& 0.54  & 0.55  & 0.56  \\ \hline
% \textbf{RobustPeriod} &  0.82  & 0.99     & 0.44  & 0.98   &  0.56  & 0.57  \\ \hline        
% \end{tabular}
% \end{table}




 

% \textbf{0.72}

% \begin{table}[!htb] % \begin{table*}[t]
% % \footnotesize 
% \centering
% %\normalsize
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \caption{Comparisons of different single-periodicity detection algorithms on CRAN data.}
% %\vspace{-0.1cm}
% \label{tab:single_period_real}
% \begin{tabular}{c||c|c|c||c|c|c|}
% \hline
% \multirow{2}{*}{Algorithms}  & \multicolumn{3}{|c||}{ CRAN dataset (82 ts) } & \multicolumn{3}{|c|}{  } \\ \cline{2-7}
%  &  $0\%$ & $2\%$ & $5\%$     &    &   &  \\ \hline
% Fisher &  0.34 & 0.39 & 0.39           &  & & \\ \hline
% findFrequency & 0.44 & 0.44 & 0.45    &   &  &  \\ \hline
% SAZED$_{opt}$ & 0.55  & 0.56 & 0.56   &  &  &   \\ \hline
% {RobustPeriod} &  0.56  & 0.57 &  0.57     &    &  &   \\ \hline
% \end{tabular}
% \end{table}










\begin{table}[!htb] % \begin{table*}[t]
\centering
\caption{Precision of different single-periodicity detection algorithms on synthetic data with different noise variance $\sigma^2_n$ and outlier ratio $\eta$, as well as the real-world dataset from CRAN.}
%\vspace{-0.1cm}
\label{tab:single_period_det}
\begin{tabular}{c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{Algorithms} & \multicolumn{4}{c|}{Synthetic Data}  & \multicolumn{2}{c|}{\multirow{2}{*}{CRAN Data}} \\ \cline{2-5}
                  & \multicolumn{2}{c|}{\!$\sigma^2_n$ \!=\! 0.1, $\eta$ \!=\! 0.01\!} & \multicolumn{2}{c|}{\!$\sigma^2_n$ \!=\! 2, $\eta$ \!=\! 0.2\!} & \multicolumn{2}{c|}{}                  \\ \cline{2-7} 
 &  0\% & 2\% & 0\%   &  2\% & 0\% & 2\% \\ \hline\hline
findFrequency   &  0 & 0&        0 &0  & 0.44 & 0.44\\ \hline
% Fisher        &  \textbf{1.0} & \textbf{1.0}        & \textbf{0.59} &0.59   &  0.34 & 0.39 \\ \hline
SAZED$_{maj}$      & 0 &  0          & 0  & 0.32   &  0.49 & 0.49 \\ \hline
SAZED$_{opt}$      & 0  & 0.96       & 0  & 0.54   & 0.55  & 0.56  \\ \hline
\textbf{RobustPeriod} &  \textbf{0.83}  & \textbf{1.0}    & \textbf{0.44}  & \textbf{0.98}   &  \textbf{0.56}  & \textbf{0.57}  \\ \hline        
\end{tabular}
\end{table}

\subsection{Experiments and Discussion on Multi-Periodicities Detection}
%\subsubsection{Synthetic Data}
To evaluate the performance of different algorithms, we generate synthetic datasets with complex patterns of length $1024$, which includes three periodic components, multiple outliers, changing trend, and noises. Specifically, we first generate three sinusoidal wave with amplitude of $1$ and period length as $20, 50, 100$. Then, we add a triangle signal with amplitude of $10$ as trend. Next, we add Gaussian noise with different variances ($\sigma_n^2=$0.1, 0.5, or 2). Then, we add different number of spikes and dips with $5$ amplitude to represent outliers (the outlier ratio $\eta=1\%$, $5\%$, or $20\%$). As an example, one synthetic data with noise $\sigma_n^2=0.5$ and outlier ratio $\eta=5\%$ are shown in Figure~\ref{fig:simdata}. 




%\subsubsection{Comparisons with Existing Algorithms}

Table~\ref{tab:simData_diffNoiseOutlier} summarizes the periodicity detection results from different algorithms under mild scenario (noise variance $\sigma_n^2=0.1$, outlier ratio $\eta=1\%$) and severe scenario ($\sigma_n^2=2$ and $\eta=20\%$). 
Note that ACF-Med and Fisher method can only detect a single period. The ACF-Med fails to detect a single period in both scenarios, whereas Fisher method detects the period of $50$ correctly in both cases. The Siegel method and Wavelet-Fisher can detect all periods quite close to the ground truth, but it also introduces some false positives. AUTOPERIOD achieves a decent performance in the mild scenario, but it is very sensitive to noises and outliers as its performance degrades significantly in the severe scenario. Also it fails to detect multiple interlaced periods. In comparison, our tfPerioid algorithm detects all the true periods accurately and robustly in both scenarios. 




\begin{table}[!htb] % \begin{table*}[t]
\centering
\footnotesize
% \tiny, \scriptsize, \footnotesize, \small, \normalsize, 
\caption{F1 scores of different Multi-periodicity detection algorithms on synthetic data with different noise variance $\sigma^2_n$ and outlier ratio $\eta$, as well as the public dataset from Yahoo.}
%\vspace{-0.1cm}
\label{tab:multi_period_det}
\begin{tabular}{c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{Algorithms} & \multicolumn{4}{c|}{Synthetic Data}  & \multicolumn{2}{c|}{\multirow{2}{*}{Yahoo-A3}} & \multicolumn{2}{c|}{\multirow{2}{*}{Yahoo-A4}} \\ \cline{2-5}
                  & \multicolumn{2}{c|}{\!\!\!$\sigma^2_n$ \!=\! 0.1, \!$\eta$ \!=\! 0.01\!\!} & \multicolumn{2}{c|}{\!\!$\sigma^2_n$ \!=\! 2, \!$\eta$ \!=\! 0.2\!\!} & \multicolumn{2}{c|}{}  & \multicolumn{2}{c|}{}                 \\ \cline{2-9} 
 &  0\% & 2\% & 0\%   &  2\% & 0\% & 2\% & 0\% & 2\% \\ \hline\hline
Siegel                   &  0.67       & 0.68& \textbf{0.83} &0.83         & 0.75 & 0.75& 0.58 & 0.58    \\ \hline
\!AUTOPERIOD\!           &  0.25       & 0.51        & 0.14  &0.34         &  0.8 & 0.8 & 0.61 & 0.6   \\ \hline
\!Wavelet-Fisher\!       &  0.5        & 0.75        & 0.48  &0.72          & 0.5  & 0.76  & 0.49& 0.73  \\ \hline
\!\textbf{RobustPeriod}\!&\textbf{0.84}&\textbf{0.96}& 0.74  &\textbf{0.93} &  \textbf{0.82} & \textbf{0.85}& \textbf{0.82} &\textbf{0.89}\\ \hline        
\end{tabular}
\end{table}

% 0.67 0.25 0.5  0.84
% 0.68 0.51 0.75 0.96
% 0.83 0.14 0.48 0.74
% 0.83 0.34 0.72 0.93

% [0.75 0.8  0.5  0.82]
% [0.75 0.8  0.76 0.85]
% [0.58 0.61 0.49 0.82]
% [0.58 0.6  0.73 0.89]



\begin{figure*}[!htb]
\centering
    \includegraphics[width=1\linewidth]{plots/multiPeriods_pre_recall_f1.pdf}
    \caption{Detailed precision, recall, and F1}
    % \caption{Five representative real-world datasets: the first three datasets contain single period with length $12, 144, 288$, respectively; the last two datasets contain double periods with lengths as $(6,12), (48,336)$, respectively.}
\label{fig:multiP_pre_recall_f1}
\end{figure*}







% mild, tol=2%
% precision_mean is [1.   0.96 0.4  1.   1.  ]
% recall_mean    is [0.33 0.32 0.96 0.95 0.95]
% f1_mean        is [0.5  0.48 0.49 0.97 0.97]
% severe,tol=2%
% precision_mean is [1.   1.   0.47 0.99 1.  ]
% recall_mean    is [0.33 0.33 0.98 0.96 0.98]
% f1_mean        is [0.5  0.5  0.56 0.98 0.99]




 


%\begin{itemize}
%    \item ACF-Med and Fisher methods can only detect single period...
%    \item Siegel and Wavelet-Fisher algorithms can obtain near the true three periods. However, they produce many false-positive results...
%    \item AutoPeriod cannot detect the period length 50, since the ACF does not have peak due to the effect of both period lengths 20 and 50. 
%    \item Both By contrast, the proposed RobustPeriod algorithm correctly detect the true three periods under both scenarios without any false-positive results.
%\end{itemize}

 

(TODO) Table~\ref{tab:YahooData} summarizes the periodicity detection results from different algorithms on Yahoo dataset A3 and A4. (Add two typical figures from Yahoo A3, A4)



% \begin{table}[!htb] % \begin{table*}[t]
% % \footnotesize 
% \centering
% %\normalsize
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \caption{Comparisons of different periodicity detection algorithms on Yahoo dataset A3 and A4. The true periods are (12,24,128).}
% %\vspace{-0.1cm}
% \label{tab:YahooData}
% \begin{tabular}{c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Algorithms}  & \multicolumn{3}{|c|}{ Yahoo A3 } & \multicolumn{3}{|c|}{ Yahoo A4 } \\ \cline{2-7}
%  &  pr & re & f1     & pr  & re & f1\\ \hline\hline
% % ACF-Med &  \textbf{1.0} & 0.33 & 0.50           &  \textbf{1.0} & 0.33 & 0.50 \\ \hline
% % Fisher &  0.96 & 0.32 & 0.48     & \textbf{1.0} & 0.33 & 0.50 \\ \hline
% Siegel & 0.66  & \textbf{0.99}& 0.75   & 0.45& \textbf{0.99}& 0.58 \\ \hline
% AUTOPERIOD & \textbf{0.99} &0.67 & 0.79           &  0.63 & 0.67& 0.60 \\  \hline
% Wavelet-Fisher  &0.41  & 0.67 & 0.50     & 0.39  &0.67 & 0.49 \\ \hline
% \textbf{RobustPeriod} &  0.89  & 0.84 &  \textbf{0.86}     &  \textbf{0.91} & 0.89& \textbf{0.90}  \\ \hline
% \end{tabular}
% \end{table}



%\subsubsection{Analysis of Intermediate Results from RobustPeriod(TODO)}

To further understand the process of how RobustPeriod detects multiple periodicities, we plot the intermediate results in Fig.~\ref{fig:tfDetail}. In Fig.~\ref{fig:tfDetail:all_level}, the first column is the wavelet coefficient, the second column is the Huber-periodogram, and the last column is the robust ACF; each row corresponds to a wavelet coefficient at a specific level. It can be observed that MODWT effectively decouples the interlaced periodicities. The Huber-periodogram and robust ACF effectively detect the periods of 20, 50, and 100 at level 4, 5, and 6, respectively. As a comparison, AUTOPERIOD cannot detect the period of $50$ as the vanilla ACF does not have peak near 50 (the vanilla ACF drops near 50 due to the strong periodicities of 20 and 100). Fig.~\ref{fig:tfDetail:WV} plots the wavelets variances at different levels. It is clear that large wavelet variances correspond to strong periodic patterns at levels 4, 5, and 6. 




\begin{figure}[!htb]
    \centering
    \subfigure[Wavelet coefficient, Huber-periodogram, and robust ACF at different level: the true period lengths 20, 50, 100 are correctly detected at level 4,5,6.]{
        \includegraphics[width=0.9\linewidth]{plots/simEx-WaveFFTACF.pdf}
        \label{fig:tfDetail:all_level}
        }
        \\ \vspace{-0.2cm}
    \subfigure[Wavelet variance at different level: the levels 4,5,6 have high wavelet variance, which also corresponds to the location of periodic components]{
        \includegraphics[width=0.9\linewidth]{plots/simEx-WaveVariance.pdf}
        \label{fig:tfDetail:WV}
        } \vspace{-0.3cm}
    \caption{Intermediate results of the RobustPeriod algorithm.}
    \label{fig:tfDetail}
\end{figure}










% %%%%% backup: only one-time run
% \begin{table}[!htb] % \begin{table*}[t]
% \footnotesize \centering
% %\normalsize
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \caption{Comparisons of different periodicity detection algorithms on synthetic data with different noises and outliers. The true periods are (20,50,100).}
% %\vspace{-0.1cm}
% \label{tab:simData_diffNoiseOutlier}
% \begin{tabular}{c|c|c}
% \hline
% \multirow{2}{*}{Algorithms}  & \multicolumn{2}{|c}{noise variance $\sigma^2_n$ \& outlier ratio $\eta$} \\ \cline{2-3}
% &  $\sigma^2_n$ = 0.1, $\eta$ = 1\% & $\sigma^2_n$ = 2, $\eta$ = 20\% \\ \hline
% %  & $\eta$ = 1\%  & $\eta$ = 20\% \\ \hline
% ACF-Med &  19  & 3\\ \hline
% Fisher &  50  & 50\\ \hline
% Siegel & (20,102,51,512,93,...) & (20 ,49,102,51,1024) \\ \hline
% AUTOPERIOD & (19,102) &    20  \\  \hline
% Wavelet-Fisher  & (20,50,102,512)  & (20, 50, 98,205,5)  \\ \hline
% {RobustPeriod} &  (20,50,100)  &  (20,50,100) \\ \hline
% \end{tabular}
% \end{table}





%\begin{itemize}
%    \item the MODWT decouples the interference of multiple periods
%    \item the combined Huber-periodogram and ACF detect the correct period 20, 50, 100 at level 4,5,6, respectively.
%    \item AutoPeriod cannot detect the period length 50, since the ACF does not have peak due to the effect of both period lengths 20 and 50. 
%    \item Both By contrast, the proposed RobustPeriod algorithm correctly detect the true three periods under both scenarios without any false-positive results.
%\end{itemize}




% \begin{table}[t] % \begin{table*}[t]
% \footnotesize \centering
% %\normalsize
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \caption{Comparisons of periodicity detection on synthetic data with different noises and outliers. The true periods are (20,50,100).}
% %\vspace{-0.1cm}
% \label{tab:simData_diffNoiseOutlier}
% \begin{tabular}{c|c|c|c}
% \hline
% \multirow{3}{*}{Algorithms}  & \multicolumn{3}{|c}{noise variance $\sigma^2_n$ \& outlier ratio $\eta$} \\ \cline{2-4}
% &  $\sigma^2_n$ = 0.1 & $\sigma^2_n$ = 0.5 & $\sigma^2_n$ = 2 \\ 
%  & $\eta$ = 1\% & $\eta$ = 5\% & $\eta$ = 20\% \\ \hline
 
% ACF-Med &  19 & 5 & 3\\ \hline
% Fisher &  50 & 50 & 50\\ \hline
% Siegel & (20,102,51,512,93,...) & (20,51,102,47,114,...)& (20 ,49,102,51,1024) \\ \hline
% AutoPeriod & (19,102) & (20,102) &   20  \\  \hline
% Wavelet-Fisher  & (20,50,102,512) & (20,50,102,410) & (20, 50, 98,205,5)  \\ \hline
% {RobustPeriod} &  (20,50,100) &  (20,50,100) &  (20,50,100) \\ \hline
% \end{tabular}
% \end{table}

% \begin{table*}[t]
% \footnotesize \centering
% %\normalsize
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \label{tab:simData_diffNoise}
% \begin{tabular}{c|c|c|c|c|c|c}
% \hline
% \multirow{3}{*}{Algorithms} & \multicolumn{3}{|c|}{noise variance} & \multicolumn{3}{|c}{noise variance $\sigma^2_n$ \& outlier ratio $\eta$} \\ \cline{2-7}
% & \multirow{2}{*}{$\sigma^2_n$ = 0.1} & \multirow{2}{*}{$\sigma^2_n$ = 0.5} & \multirow{2}{*}{$\sigma^2_n$ = 2} & $\sigma^2_n$ = 0.1 & $\sigma^2_n$ = 0.5 & $\sigma^2_n$ = 2 \\ 
% & & & & $\eta$ = 1\% & $\eta$ = 5\% & $\eta$ = 20\% \\ \hline
% DFT-Fisher & 512 & 512 & 512 & 512 & 512 & 512\\ \hline
% M-DFT-Fisher & 512 & 512 & 512 & 512 & 512 & 512\\ \hline
% ACF-Median & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
% {DFT-Th} & 20, 51, 102, 512 & 20, 102, 512 & 20, 102, 512 &  20, 102, 512 &  20, 51, 102, 512 &  20, 512 \\ \hline
% {M-DFT-Th} & 20, 256, 512 & 20, 256, 512 & 20, 256, 512 &  20, 256, 512 &  256, 512 &   256, 512  \\  \hline
% AutoPeriod & 20, 100 & 20, 100 & 20, 99 & 20, 100 & 20, 100& 20  \\ \hline
% RobustPeriod & 20, 50, 100 &  20, 50, 100 &  20, 50, 100 &  20, 50, 100 &  20, 50, 100 &  20, 50, 100 \\ \hline
% \end{tabular}
% \caption{bbbb}
% \end{table*}



%%%%% 
% \begin{figure}[!htb] 
%     \centering
%     \includegraphics[width=0.9\linewidth]{plots/simEx-removeTrend.pdf}
%     \caption{BBB From top to bottom: the three sine waves with different periods; the summation of the three sine waves; simulated noise, $20$ spike \& dip outliers, and trend with both slow and abrupt changes (orange line); the final synthetic data.}
% \label{fig: sec4-sine-data}
% \end{figure}










% \subsection{Comparisons on Periodicity Detection with Multi-Seasons}


% \subsubsection{Experiment Results on Synthetic Data}
% We summarize the results of periodicity detection of DFT-Periodogram, AUTOPERIOD, and our proposed approach in Table~\ref{table:period-result}. For the result comparison, each scheme outputs the the top-3 and top-2 period lengths for synthetic sine/square and real data respectively. The last row of the table is the ``ground truth". It can be seen that our method achieves the best performance among all the schemes. 

% \begin{table}%\label{table:period-result}
% \begin{center}
%   \begin{tabular}{ l | l | l | l}
%     \hline
%         & Sine wave & Square wave & Real data \\ \hline 
%     DFT-Periodogram & (672,168,1792) & (672,168,24) & (24,616) \\ \hline 
%     AutoPeriod & (672,168,25) & (672,168,24) & (24,360) \\\hline
%     \textbf{RobustPeriod} & \textbf{(672,168,24)} & \textbf{(672,168,24)} & \textbf{(24,168)} \\\hline
%     Ground truth & (672,168,24) & (672,168,24) & (24,168) \\\hline
%   \end{tabular}
%   \caption{Summary of periodicity detection results.}
% \label{table:period-result}
% \end{center}
% \end{table}

% To better understand the detection results of each methods, the Periodogram and ACF of the real-world dataset with two seasons are plotted in Figure~\ref{fig: sec4-sine-data-period-acf}. The true periods of the dataset are $(24,168)$, which corresponds to the frequency points at position $(77, 11)$. It can be seen that both AUTOPERIOD and our proposed method capture the frequency point at position $77$ correctly. However, the AUTOPERIOD is difficult to locate the true frequency point at position $11$ while our method can also capture the true frequency point at position $11$. Furthermore, the ACF figure of our method is also easier than AUTOPERIOD to find the peak points corresponding to the periods.

% The left side shows the Periodogram and ACF from DFT-Periodogram and AUTOPERIOD. It can be seen that the Periodogram is contaminated by    

% the periodogram and ACF plots are generated by both baseline algorithms and our methods. When examining the plots closely, we found that with our approach, the true second periodicity 168 is captured as candidate in the periodogram, while the FFT method fails to do that. See things about the ACF plots.

% \begin{figure}[!htb]
%     \includegraphics[width=1.0\linewidth]{plots/sec4-sine-data-period-acf-new.pdf}
%     \caption{Periodogram and ACF results from AUTOPERIOD (left-side) and our proposed method (right-side). The AUTOPERIOD is hard to locate the true frequency point at position $11$ in Periodogram, and the ACF is also not as good as our proposed method.}
% \label{fig: sec4-sine-data-period-acf}
% \end{figure}




\begin{table}[!htb] % \begin{table*}[t]
% \footnotesize 
\centering
%\normalsize
% \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
\caption{Ablation studies of the proposed RobustTrend  on synthetic data with different noise variance $\sigma^2_n$ and outlier ratio $\eta$. The true periods are (20,50,100).}
%\vspace{-0.1cm}
\label{tab:Ablation}
\begin{tabular}{c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Algorithms}  & \multicolumn{3}{|c|}{ $\sigma^2_n$ = 0.1, $\eta$ = 1\% } & \multicolumn{3}{|c|}{ $\sigma^2_n$ = 2, $\eta$ = 20\% } \\ \cline{2-7}
 &  pr & re & f1     & pr  & re & f1\\ \hline\hline
% ACF-Med &  0 & 0 & 0           & 0 &0 & 0\\ \hline
% Fisher &  \textbf{1.0} & 0.33 & 0.50     & \textbf{0.82} &0.27 &0.41 \\ \hline
Huber-ACF-Med     & \textbf{1}     & 0.33   & 0.5         & \textbf{1}  & 0.33& 0.5 \\ \hline
Huber-Fisher      & 0.96           &0.32   & 0.48         &  \textbf{1}  & 0.33& 0.5 \\  \hline
Huber-Siegel-ACF  &0.4    & \textbf{0.96}  & 0.49         & 0.47         &\textbf{0.98} & 0.56 \\ \hline
NR-RobustPeriod   &\textbf{1}      & 0.95  & \textbf{0.97} & 0.99         &0.96 & 0.98 \\ \hline
\textbf{RobustPeriod} &\textbf{1}  & 0.95  &\textbf{0.97}  &  \textbf{1} & \textbf{0.98}& \textbf{0.99}  \\ \hline
\end{tabular}
\end{table}







\begin{table*}[!htb]
\small 
\centering
% \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
\caption{Comparisons of different periodicity detection algorithms on five real-world datasets.}
\label{tab:realData_diff_algs}
\begin{tabular}{c|c|c|c|c|c}
\hline
% \multirow{2}{*}{Algorithms} & Data-1 & Data-2 & Data-3 & Data-4 & Data-5 \\
% & (12) & (144) & (288) & (6,12) & (48,336) \\ \hline 
Algorithms & Data-1, \textbf{T=12} & Data-2, \textbf{T=144} & Data-3, \textbf{T=288} & Data-4, \textbf{T=(6,12)} & Data-5, \textbf{T=(48,336)} \\\hline \hline
% \textbf{True Periods} & \textbf{12} & \textbf{144} & \textbf{288} & \textbf{(6,12)} & \textbf{(48,336)} \\ \hline
% ACF-Med & 12 & 144 & 283 & 6 & 48 \\ \hline
% Fisher & 12 & 1024 & 293 & NA & 48 \\ \hline
Siegel & (12,256,4) & (146,256,410,...) & (293,273,141,...) & (6,12) & (48,341,171,...) \\ \hline
% \multirow{4}{*}{Siegel} & 12 & 1024 & 2048 & 6 & 48 \\ 
% & 128 & 603 & 293 & 12 & 341 \\ 
% &  & 512 & \dots &   & 49 \\ 
% &  & \dots &   &  & \dots \\ \hline
% \multirow{4}{*}{AutoPeriod} & 12 & 293 & 2048 & 6 & 48 \\ 
% & 128 & 146 & 293 & 12 & 341 \\ 
% &  & 1024 & 256 &   & 49 \\ 
% &  & \dots & \dots &  & \dots \\ \hline
AUTOPERIOD & 12 & 145 & (288,276,327,...) & (6,12) & (48,53,43,...) \\ \hline
Wavelet-Fisher & (12,6,51,...) & (146,372,48,...) & (292,585,144) & (6,12) & (48,341,12,...) \\ \hline\hline
% \multirow{4}{*}{AutoPeriod} & 12 & 0 & 288 & 6 & 48 \\ 
% &   &  & 1441 & 12 & 53 \\ 
% &   &   & 1146 &  & 43 \\ 
% &   &   & \dots &  & 55 \\ \hline
% RobustPeriod & 12 & 144 & 288 & (6,12) & (48,340) \\ \hline

Huber-ACF-Med & 12 & 144 & 288 & 6 & 48 \\ \hline
% \multirow{4}{*}{Huber-Fisher} & 12 & 1024 & 2048 & 6 & 48 \\ 
% & 128 & 603 & 293 & 12 & 341 \\ 
% &  & 512 & \dots &   & 49 \\ 
% &  & \dots &   &  & \dots \\ \hline
Huber-Fisher & 12 & 146 & 293 & NA & 48 \\ \hline
% \multirow{4}{*}{Huber-Siegel-ACF} & 12 & 293 & 2048 & 6 & 48 \\ 
% & 128 & 146 & 293 & 12 & 341 \\ 
% &  & 1024 & 256 &   & 49 \\ 
% &  & \dots & \dots &  & \dots \\ \hline
Huber-Siegel-ACF & (12,168,156,...) & (144,432,288,...) & (288,864,576,...) & (6,12) & (48,336,384) \\ \hline
NR-RobustPeriod & 12 & NA & (286,287) & (6,12) & (48,339) \\ \hline
\textbf{RobustPeriod} & 12 & 144 & 288 & (6,12) & (48,340) \\ \hline
\end{tabular}
% \caption{Comparison}
\end{table*}


% \vspace{-0.1cm}



% \begin{table*}[htb]
% \footnotesize \centering 
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \caption{Different components analysis for RobustPeriod on real-world datasets.}
% \label{tab:realData_RobustPeriod_components}
% \begin{tabular}{c|c|c|c|c|c}
% \hline
% % \multirow{2}{*}{Algorithms} & Data-1 & Data-2 & Data-3 & Data-4 & Data-5 \\
% % & (12) & (144) & (288) & (6,12) & (48,336) \\ \hline 
% Algorithms & Data-1, \textbf{T=12} & Data-2, \textbf{T=144} & Data-3, \textbf{T=288} & Data-4, \textbf{T=(6,12)} & Data-5, \textbf{T=(48,336)} \\\hline 

% Huber-ACF-Med & 12 & 144 & 288 & 6 & 48 \\ \hline
% % \multirow{4}{*}{Huber-Fisher} & 12 & 1024 & 2048 & 6 & 48 \\ 
% % & 128 & 603 & 293 & 12 & 341 \\ 
% % &  & 512 & \dots &   & 49 \\ 
% % &  & \dots &   &  & \dots \\ \hline
% Huber-Fisher & 12 & 146 & 293 & NA & 48 \\ \hline
% % \multirow{4}{*}{Huber-Siegel-ACF} & 12 & 293 & 2048 & 6 & 48 \\ 
% % & 128 & 146 & 293 & 12 & 341 \\ 
% % &  & 1024 & 256 &   & 49 \\ 
% % &  & \dots & \dots &  & \dots \\ \hline
% Huber-Siegel-ACF & (12,168,156,...) & (144,432,288,...) & (288,864,576,...) & (6,12) & (48,336,384) \\ \hline
% NR-RobustPeriod & 12 & NA & (286,287) & (6,12) & (48,339) \\ \hline
% % \multirow{4}{*}{AutoPeriod} & 12 & 0 & 288 & 6 & 48 \\ 
% % &   &  & 1441 & 12 & 53 \\ 
% % &   &   & 1146 &  & 43 \\ 
% % &   &   & \dots &  & 55 \\ \hline
% RobustPeriod & 12 & 144 & 288 & (6,12) & (48,340) \\ \hline
% \end{tabular}
% % \caption{Comparison}
% \end{table*}







\subsection{Experiments and Discussion on Real-world Data}
%\subsubsection{Real-world Data}
We adopt five representative real-world datasets as shown in Fig.~\ref{fig:realDatasets}. The first three datasets (workforce, trading volume, and file exchange count) contain single period with length $12, 144, 288$, respectively. The last two datasets (electricity usage) contain double periods with lengths as $(6,12), (48,336)$, respectively. The first, fourth, and fifth datasets are from public tsdl library\footnote{Time Series Data Library. v0.1.0. https://pkg.yangzhuoranyang.com/tsdl/}. The second and third datasets are collected from one cloud computing company. 
% We normalized these two datasets for the purpose of anonymization. 

\begin{figure}[!htb]
\centering
    \includegraphics[width=0.75\linewidth]{plots/realdata.pdf}
    \caption{Real-world datasets: the first 3 datasets contain single period while the last 2 datasets have double periods.}
    % \caption{Five representative real-world datasets: the first three datasets contain single period with length $12, 144, 288$, respectively; the last two datasets contain double periods with lengths as $(6,12), (48,336)$, respectively.}
\label{fig:realDatasets}
\end{figure}




%\subsubsection{Comparisons with Existing Algorithms(TODO)}

Table~\ref{tab:realData_diff_algs} summarizes the periodicity detection results from different algorithms on the five real-world datasets. The Fisher method fails to detect the periodicities on Data-2 and Data-4. The failure on Data-2 is due to the high amplitude in one period. For Data-4, the complex trend and outliers make Fisher fail. Compared to Fisher, Siegel and Wavelet-Fisher can detect multiple periods, but they tend to introduce too many false alarms. AUTOPERIOD also has many false positive on Data-3 and Data-5, and it misses the period 336 on Data-5. By contrast, our RobustPeriod algorithm correctly detects the true periods on all five datasets (only on Data-5 the detected period is 340 while the truth is 336). 
 
%\begin{itemize}
%    \item ACF-Med and Fisher can only detect single dominant period. For Data-2 due to high amplitude only within one period interval, Fisher fails; for Data-4, due to complex trend and outlier, Fisher also fails;
%    \item Siegel has many false positive 
%    \item AutoPeriod also has many false positive at Data-3 and Data-5, and it missed the period 336. Wavelet-Fisher also has many false positive.
%    \item Both By contrast, the proposed RobustPeriod algorithm correctly detect the true  periods in all five datasets (only Data-5, there is minor error the the longer period 336).
%\end{itemize}






% \begin{table}[htb]
% \footnotesize \centering
% % \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, and \Huge.
% \caption{Excution time cmp}
% %\vspace{-0.1cm}
% \label{tab:changePoint-comparison-synthetic}
% \begin{tabular}{c|c|c|c|c}
% \hline
% Algorithm & N = 256 & N = 512 & N = 1024 & N = 2048 \\ \hline
% Auto Period & 12.8ms & 16.8ms & 22.7ms & 47.2ms \\ \hline
% RobustPeriod & \multirow{2}{*}{1.96s} & \multirow{2}{*}{5.09s} & \multirow{2}{*}{12.9s} & \multirow{2}{*}{37s} \\ 
% (with periodicity) & & & &  \\ \hline
% RobustPeriod (non-robust) & \multirow{2}{*}{4.36ms} & \multirow{2}{*}{5.69ms} & \multirow{2}{*}{7.91ms} & \multirow{2}{*}{16.1ms} \\ 
% (with M-periodicity) & & & &  \\ \hline
% \end{tabular}
% \end{table}

 

%\subsubsection{Analysis of Different Components of RobustPeriod(TODO)}
% (Ablation studies)
We further evaluate the contribution of different components of the RobustPeriod algorithm for periodicity detection. Specifically, we compare the performance of RobustPeriod with the following revisions:
\begin{itemize}
    \item \textbf{Huber-ACF-Med}: It is based on the previous \textit{ACF-Med} by using Huber-periodogram and robust ACF.
    \item \textbf{Huber-Fisher}: This algorithm has the same procedure as the \textit{Fisher} except that the vanilla periodogram is replaced by Huber-periodogram.
    \item \textbf{Huber-Siegel-ACF}: This algorithm also adopt Huber-periodogram when finding multiple period candidates using Siegel's test. Then, the candidates are validated by checking if they are located near the peaks of ACF as in AUTOPERIOD.
    \item \textbf{NR-RobustPeriod}: This one is non-robust version of RobustPeriod by using vanilla periodogram and ACF while the structure is the same as RobustPeriod.
\end{itemize}

Table~\ref{tab:realData_RobustPeriod_components} summarizes the periodicity detection results of the aforementioned revisions on the five real-world datasets. Our first observation is that Huber-periodogram significantly improves the detection performance. Both Huber-ACF-Med and Huber-Fisher achieve better performance than ACF-Med and Fisher, respectively. For example, on Data-3, Huber-ACF-Med obtains the accurate period length 288, while ACF-Med gets 283; on Data-2, Huber-Fisher obtains near accurate period length 146, while Fisher get the wrong result 1024. Secondly, the Siege's test is not ideal for multiple periodicity detection. Huber-Siegel-ACF achieves better performance due to Huber-periodogram, but it still cannot decouple the interlaced multiple periodicities. Lastly, the pipeline of the proposed RobustPeriod still shines as  NR-RobustPeriod can still obtain the correct results in most cases. 



(TODO) refer to Fig.~\ref{fig:Peri_ACF_Ori}, Fig.~\ref{fig:Peri_ACF_LAD}, and Fig.~\ref{fig:Peri_ACF_Huber}

\begin{figure}[!htb] 
    \centering
    \includegraphics[width=0.9\linewidth]{plots/Peri_ACF_Ori.pdf}
    \caption{Ori Periodogram and ACF }
\label{fig:Peri_ACF_Ori}
\vspace{-0.2cm}
\end{figure}
% period = 24  , ori_len=102, len(data_pad)=204, peri->peak at 8,9
% len(data_pad)/8,len(data_pad)/9 = (25.5, 22.67)
\begin{figure}[!htb]
    \centering
    \subfigure[LAD Periodogram and ACF]{
        \includegraphics[width=0.9\linewidth]{plots/Peri_ACF_LAD.pdf}
        \label{fig:Peri_ACF_LAD}
        }
        \\ \vspace{-0.2cm}
    \subfigure[Huber Periodogram and ACF]{
        \includegraphics[width=0.9\linewidth]{plots/Peri_ACF_Huber.pdf}
        \label{fig:Peri_ACF_Huber}
        } \vspace{-0.3cm}
    \caption{Comparisons of LAD and Huber based Periodogram and ACF}
    \label{fig:Peri_ACF_LADHuber}
\end{figure}





%\begin{itemize}
%    \item Huber-ACF-Med has better performance than ACF-Med due to our proposed Huber-periodogram based ACF. For example in Data-3, Huber-ACF-Med obtains the accurate period length 288, while ACF-Med gets 283.
%    \item Huber-Fisher has better performance than Fisher due to our proposed Huber-periodogram, For example in Data-2, Huber-Fisher obtains near accurate period length 146, while Fisher get the wrong result 1024.
%    \item Huber-Siegel-ACF also has minor improvement than Siegel (e.g., less false positive in Data-5), but its performance is still not good since it cannot decouple the interference of multiple periods.
%    \item NR-RobustPeriod employs the structure of RobustPeriod so it can obtain the correct results in most of cases. Only in Data-2, NR-RobustPeriod cannot detect the correct results due to...
    
%    \item Both By contrast, the proposed RobustPeriod algorithm correctly detect the true periods in all five datasets (only Data-5, there is minor error the the longer period 336).
%\end{itemize}








% \begin{figure}[!htb]
%  \centering
 
 
%     \includegraphics[width=0.8\linewidth]{plots/simEx-WaveFFTACF.pdf}
%     \caption{AAA From top to bottom: the real-world dataset with two seasonal patterns (daily and weekly seasons); the updated real-world dataset by adding a abrupt trend change, one spike outlier, one dip outlier, and pattern outlier spanning one day.}
% \label{fig: 5-data-generating}
% \end{figure}

% \begin{figure}[!htb]
%     \includegraphics[width=0.9\linewidth]{plots/simEx-WaveVariance.pdf}
%     \caption{BBB}
% \label{fig: 5-data-generating}
% \end{figure}





% \begin{figure}[!htb]
%     \centering
%     \subfigure[Synthetic Data]{
%         \includegraphics[width=0.9\linewidth]{figs/synthetic-raw.pdf} 
%         \label{fig:dataset-synthetic}
%         }
%         \\\vspace{-0.1cm}
%     \subfigure[Real-world Data]{
%         \includegraphics[width=0.9\linewidth]{figs/real-raw.pdf}
%         \label{fig:dataset-real}
%         } \vspace{-0.3cm}
%     \caption{Synthetic and real-world data used for the experiment.}
%     \label{fig:dataset}
% \end{figure}
